Sharp Deviations Bounds for Dirichlet Weighted Sums with Application to analysis of Bayesian algorithms

In this work, we derive sharp non-asymptotic deviation bounds for weighted sums of Dirichlet random variables. These bounds are based on a novel integral representation of the density of a weighted Dirichlet sum. This representation allows us to obtain a Gaussian-like approximation for the sum distribution using geometry and complex analysis methods. Our results generalize similar bounds for the Beta distribution obtained in the seminal paper Alfers and Dinges [1984]. Additionally, our results can be considered a sharp non-asymptotic version of the inverse of Sanov's theorem studied by Ganesh and O'Connell [1999] in the Bayesian setting. Based on these results, we derive new deviation bounds for the Dirichlet process posterior means with application to Bayesian bootstrap. Finally, we apply our estimates to the analysis of the Multinomial Thompson Sampling (TS) algorithm in multi-armed bandits and significantly sharpen the existing regret bounds by making them independent of the size of the arms distribution support.

==> source/upper_bound.tex <==
\section{Upper bound}
The proof of upper bound generalizes proof of \cite{baudry2021optimality} to non-integer parameters using exactly the same technique; see also \cite{riou20a}.
\begin{theorem}[Upper bound]\label{thm:upper_bound_dbc}
    For any $\alpha = (\alpha_0, \alpha_1, \ldots, \alpha_m) \in \R_{++}^{m+1}$ define  $\up \in \simplex_{m}$ such that $\up(\ell) = \alpha_\ell/\ualpha, \ell = 0, \ldots, m$, where $\ualpha = \sum_{j=0}^m \alpha_j$. Then for any $f \colon \{0,\ldots,m\} \to [0,b]$ and $0 < \mu < b$ and
  \[
        \P_{w\sim \Dir(\alpha)} [wf \geq \mu] \leq \exp(-\ualpha \Kinf(\up,\mu, f)).
  \]
\end{theorem}
\begin{proof}
    The statement is trivial for $\mu \leq \up f$ since $\Kinf(\up,\mu, f) = 0$. Assume that $\mu > \up f$. It is well know fact that $w \sim \Dir(\alpha)$ may be represented as follows
  \[
        w \triangleq \left( \frac{Y_0}{V_m}, \frac{Y_1}{V_m}, \ldots, \frac{Y_m}{V_m} \right),
  \]
  where $Y_\ell \mysim \Gamma(\alpha_\ell, 1), \ell = 0, \ldots, m$ and $V_m = \sum_{\ell=0}^m Y_\ell$. Let us fix $\lambda \in [0, 1/(b - u))$ and proceed by the changing of measure argument
  \begin{align*}
        \PP{wf \geq \mu} &= \PP{ \sum_{\ell=0}^m Y_\ell f(\ell) \geq \sum_{\ell = 0}^m Y_\ell \mu } = \E_{Y_\ell \mysim \Gamma(\alpha_\ell, 1)}\left[ \ind\left\{ \sum_{\ell=0}^m Y_\ell(f(\ell) - \mu) \geq 0 \right\} \right] \\
        &= \E_{\hat{Y}_\ell \mysim \Gamma(\alpha_\ell, 1 - \lambda(f(\ell) - \mu))}\left[ \ind\left\{ \sum_{\ell=0}^m \hat{Y}_\ell(f(\ell) - \mu) \geq 0 \right\} \prod_{\ell=0}^m \frac{\exp(-\lambda \hat{Y}_{\ell} (f(\ell) - \mu))}{(1 - \lambda(f(\ell) - \mu))^{\alpha_\ell}} \right] \\
        &= \exp\left( - \sum_{\ell=0}^m \alpha_{\ell} \log(1 - \lambda(f(\ell) - \mu)) \right)  \\
        &\qquad \cdot \E_{\hat{Y}_\ell \mysim \Gamma(\alpha_\ell, 1 - \lambda(f(\ell) - \mu))}\left[ \ind\left\{ \sum_{\ell=0}^m \hat{Y}_\ell(f(\ell) - \mu) \geq 0 \right\} \rme^{-\lambda \sum_{\ell=0}^m \hat{Y}_{\ell} (f(\ell) - \mu)}\right] \\
        &\leq \exp\left( -\ualpha \sum_{\ell=0}^m \up_{\ell} \log(1 - \lambda(f(\ell) - \mu)) \right) = \exp\left( -\ualpha \E_{X \sim \up}\left[ \log(1 - \lambda(f(X) - \mu) \right] \right).
  \end{align*}
  
   Since the previous inequality is true for all $\lambda \in[0,1/(b-\mu))$, then the variational formula (Lemma~\ref{lem:var_form_Kinf}) allows to conclude
   \begin{align*}  
        \P_{w\sim \Dir(\alpha)} [w f\geq \mu] &\leq  \exp\left(-\ualpha\sup_{\lambda \in[0,1/(b-\mu))}\E_{X \sim \up}\left[ \log(1 - \lambda(f(X) - \mu) \right]\right) \\
        &= \exp(-\ualpha \Kinf(\up,\mu, f)).
    \end{align*}
\end{proof}

